Non-perturbative Renormalization Constants using Ward Identities

We extend the application of axial Ward identities to calculate $b_A, b_P$ and $b_T$, coefficients that give the mass dependence of the renormalization constants of the corresponding bilinear operators in the quenched theory. The extension relies on using operators with non-degenerate quark masses. It allows a complete determination of the O(a) improvement coefficients for bilinears in the quenched approximation using Ward Identities alone. Only the scale dependent normalization constants $Z_P^0$ (or $Z_S^0$) and $Z_T$ are undetermined. We present results of a pilot numerical study using hadronic correlators.

==> Makefile <==
# %auto-ignore
All: paper.ps

.SILENT:
paper.ps : paper.dvi fig1b.ps fig2.ps
	dvips -z -o $@ paper.dvi

paper.dvi : paper.tex fig1b.ps fig2.ps
	latex paper.tex
	if grep -i -q rerun paper.log ; then latex paper.tex; fi
	if grep -i -q rerun paper.log ; then latex paper.tex; fi
	if grep -i -q rerun paper.log ; then echo \
		Stupid latex tells me to rerun. Giving up.; fi
fig1.ps: fig1.ax
fig1b.ps: fig1b.ax
fig2.ps: fig2.ax
%.ps : %.ax
	xyplot $< | /usr/local/bin/plot2ps > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" -e 's/useclippath true def/useclippath false def/' \
	$@.tmp > $@ 
	rm -f $@.tmp
submission: submission.uu;
submission.uu: Makefile paper.tex \
	    fig1.ax fig1b.ax fig1b.ps fig2.ax fig2.ps espcrc2.sty
	rm submission.uu
	(echo .; \
	 echo Makefile paper.tex \
	    fig1.ax fig1b.ax fig1b.ps fig2.ax fig2.ps espcrc2.sty; \
	 echo submission) | uufiles -gz -9

